3D-GOI: 3D GAN Omni-Inversion for Multifaceted and Multi-object Editing

The current GAN inversion methods typically can only edit the appearance and shape of a single object and background while overlooking spatial information. In this work, we propose a 3D editing framework, 3D-GOI, to enable multifaceted editing of affine information (scale, translation, and rotation) on multiple objects. 3D-GOI realizes the complex editing function by inverting the abundance of attribute codes (object shape/appearance/scale/rotation/translation, background shape/appearance, and camera pose) controlled by GIRAFFE, a renowned 3D GAN. Accurately inverting all the codes is challenging, 3D-GOI solves this challenge following three main steps. First, we segment the objects and the background in a multi-object image. Second, we use a custom Neural Inversion Encoder to obtain coarse codes of each object. Finally, we use a round-robin optimization algorithm to get precise codes to reconstruct the image. To the best of our knowledge, 3D-GOI is the first framework to enable multifaceted editing on multiple objects. Both qualitative and quantitative experiments demonstrate that 3D-GOI holds immense potential for flexible, multifaceted editing in complex multi-object scenes.Our project and code are released at https://3d-goi.github.io .

==> main_bbl.tex <==
\begin{thebibliography}{10}
\providecommand{\url}[1]{\texttt{#1}}
\providecommand{\urlprefix}{URL }
\providecommand{\doi}[1]{https://doi.org/#1}

\bibitem{abdal2019image2stylegan}
Abdal, R., Qin, Y., Wonka, P.: Image2stylegan: How to embed images into the stylegan latent space? In: Proceedings of the IEEE/CVF International Conference on Computer Vision. pp. 4432--4441 (2019)

\bibitem{alaluf2022hyperstyle}
Alaluf, Y., Tov, O., Mokady, R., Gal, R., Bermano, A.: Hyperstyle: Stylegan inversion with hypernetworks for real image editing. In: Proceedings of the IEEE/CVF conference on computer Vision and pattern recognition. pp. 18511--18521 (2022)

\bibitem{arad2021compositional}
Arad~Hudson, D., Zitnick, L.: Compositional transformers for scene generation. Advances in Neural Information Processing Systems  \textbf{34},  9506--9520 (2021)

\bibitem{bau2019seeing}
Bau, D., Zhu, J.Y., Wulff, J., Peebles, W., Strobelt, H., Zhou, B., Torralba, A.: Seeing what a gan cannot generate. In: Proceedings of the IEEE/CVF International Conference on Computer Vision. pp. 4502--4511 (2019)

\bibitem{bhattarai2023triplanenet}
Bhattarai, A.R., Nie{\ss}ner, M., Sevastopolsky, A.: Triplanenet: An encoder for eg3d inversion. arXiv preprint arXiv:2303.13497  (2023)

\bibitem{brock2018large}
Brock, A., Donahue, J., Simonyan, K.: Large scale gan training for high fidelity natural image synthesis. arXiv preprint arXiv:1809.11096  (2018)

\bibitem{chan2022efficient}
Chan, E.R., Lin, C.Z., Chan, M.A., Nagano, K., Pan, B., De~Mello, S., Gallo, O., Guibas, L.J., Tremblay, J., Khamis, S., et~al.: Efficient geometry-aware 3d generative adversarial networks. In: Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition. pp. 16123--16133 (2022)

\bibitem{deng2019arcface}
Deng, J., Guo, J., Xue, N., Zafeiriou, S.: Arcface: Additive angular margin loss for deep face recognition. In: Proceedings of the IEEE/CVF conference on computer vision and pattern recognition. pp. 4690--4699 (2019)

\bibitem{deng2022learning}
Deng, Y., Wang, B., Shum, H.Y.: Learning detailed radiance manifolds for high-fidelity and 3d-consistent portrait synthesis from monocular image. arXiv preprint arXiv:2211.13901  (2022)

\bibitem{goodfellow2020generative}
Goodfellow, I., Pouget-Abadie, J., Mirza, M., Xu, B., Warde-Farley, D., Ozair, S., Courville, A., Bengio, Y.: Generative adversarial networks. Communications of the ACM  \textbf{63}(11),  139--144 (2020)

\bibitem{he2020momentum}
He, K., Fan, H., Wu, Y., Xie, S., Girshick, R.: Momentum contrast for unsupervised visual representation learning. In: Proceedings of the IEEE/CVF conference on computer vision and pattern recognition. pp. 9729--9738 (2020)

\bibitem{he2016deep}
He, K., Zhang, X., Ren, S., Sun, J.: Deep residual learning for image recognition. In: Proceedings of the IEEE conference on computer vision and pattern recognition. pp. 770--778 (2016)

\bibitem{ho2020denoising}
Ho, J., Jain, A., Abbeel, P.: Denoising diffusion probabilistic models. Advances in neural information processing systems  \textbf{33},  6840--6851 (2020)

\bibitem{huh2020transforming}
Huh, M., Zhang, R., Zhu, J.Y., Paris, S., Hertzmann, A.: Transforming and projecting images into class-conditional generative networks. In: Computer Vision--ECCV 2020: 16th European Conference, Glasgow, UK, August 23--28, 2020, Proceedings, Part II 16. pp. 17--34. Springer (2020)

\bibitem{johnson2017clevr}
Johnson, J., Hariharan, B., Van Der~Maaten, L., Fei-Fei, L., Lawrence~Zitnick, C., Girshick, R.: Clevr: A diagnostic dataset for compositional language and elementary visual reasoning. In: Proceedings of the IEEE conference on computer vision and pattern recognition. pp. 2901--2910 (2017)

\bibitem{karras2017progressive}
Karras, T., Aila, T., Laine, S., Lehtinen, J.: Progressive growing of gans for improved quality, stability, and variation. arXiv preprint arXiv:1710.10196  (2017)

\bibitem{karras2019style}
Karras, T., Laine, S., Aila, T.: A style-based generator architecture for generative adversarial networks. In: Proceedings of the IEEE/CVF conference on computer vision and pattern recognition. pp. 4401--4410 (2019)

\bibitem{karras2020analyzing}
Karras, T., Laine, S., Aittala, M., Hellsten, J., Lehtinen, J., Aila, T.: Analyzing and improving the image quality of stylegan. In: Proceedings of the IEEE/CVF conference on computer vision and pattern recognition. pp. 8110--8119 (2020)

\bibitem{ko20233d}
Ko, J., Cho, K., Choi, D., Ryoo, K., Kim, S.: 3d gan inversion with pose optimization. In: Proceedings of the IEEE/CVF Winter Conference on Applications of Computer Vision. pp. 2967--2976 (2023)

\bibitem{krizhevsky2017imagenet}
Krizhevsky, A., Sutskever, I., Hinton, G.E.: Imagenet classification with deep convolutional neural networks. Communications of the ACM  \textbf{60}(6),  84--90 (2017)

\bibitem{lan2023self}
Lan, Y., Meng, X., Yang, S., Loy, C.C., Dai, B.: Self-supervised geometry-aware encoder for style-based 3d gan inversion. In: Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition. pp. 20940--20949 (2023)

\bibitem{lin2023componerf}
Lin, Y., Bai, H., Li, S., Lu, H., Lin, X., Xiong, H., Wang, L.: Componerf: Text-guided multi-object compositional nerf with editable 3d scene layout. arXiv preprint arXiv:2303.13843  (2023)

\bibitem{metzer2022latent}
Metzer, G., Richardson, E., Patashnik, O., Giryes, R., Cohen-Or, D.: Latent-nerf for shape-guided generation of 3d shapes and textures. arXiv preprint arXiv:2211.07600  (2022)

\bibitem{mildenhall2021nerf}
Mildenhall, B., Srinivasan, P.P., Tancik, M., Barron, J.T., Ramamoorthi, R., Ng, R.: Nerf: Representing scenes as neural radiance fields for view synthesis. Communications of the ACM  \textbf{65}(1),  99--106 (2021)

\bibitem{nguyen2019hologan}
Nguyen-Phuoc, T., Li, C., Theis, L., Richardt, C., Yang, Y.L.: Hologan: Unsupervised learning of 3d representations from natural images. In: Proceedings of the IEEE/CVF International Conference on Computer Vision. pp. 7588--7597 (2019)

\bibitem{nguyen2020blockgan}
Nguyen-Phuoc, T.H., Richardt, C., Mai, L., Yang, Y., Mitra, N.: Blockgan: Learning 3d object-aware scene representations from unlabelled images. Advances in neural information processing systems  \textbf{33},  6767--6778 (2020)

\bibitem{niemeyer2021giraffe}
Niemeyer, M., Geiger, A.: Giraffe: Representing scenes as compositional generative neural feature fields. In: Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition. pp. 11453--11464 (2021)

\bibitem{perarnau2016invertible}
Perarnau, G., Van De~Weijer, J., Raducanu, B., {\'A}lvarez, J.M.: Invertible conditional gans for image editing. arXiv preprint arXiv:1611.06355  (2016)

\bibitem{poole2022dreamfusion}
Poole, B., Jain, A., Barron, J.T., Mildenhall, B.: Dreamfusion: Text-to-3d using 2d diffusion. arXiv preprint arXiv:2209.14988  (2022)

\bibitem{richardson2021encoding}
Richardson, E., Alaluf, Y., Patashnik, O., Nitzan, Y., Azar, Y., Shapiro, S., Cohen-Or, D.: Encoding in style: a stylegan encoder for image-to-image translation. In: Proceedings of the IEEE/CVF conference on computer vision and pattern recognition. pp. 2287--2296 (2021)

\bibitem{russakovsky2015imagenet}
Russakovsky, O., Deng, J., Su, H., Krause, J., Satheesh, S., Ma, S., Huang, Z., Karpathy, A., Khosla, A., Bernstein, M., et~al.: Imagenet large scale visual recognition challenge. International journal of computer vision  \textbf{115},  211--252 (2015)

\bibitem{schwarz2020graf}
Schwarz, K., Liao, Y., Niemeyer, M., Geiger, A.: Graf: Generative radiance fields for 3d-aware image synthesis. Advances in Neural Information Processing Systems  \textbf{33},  20154--20166 (2020)

\bibitem{tov2021designing}
Tov, O., Alaluf, Y., Nitzan, Y., Patashnik, O., Cohen-Or, D.: Designing an encoder for stylegan image manipulation. ACM Transactions on Graphics (TOG)  \textbf{40}(4),  1--14 (2021)

\bibitem{wang2022high}
Wang, T., Zhang, Y., Fan, Y., Wang, J., Chen, Q.: High-fidelity gan inversion for image attribute editing. In: Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition. pp. 11379--11388 (2022)

\bibitem{wei2022e2style}
Wei, T., Chen, D., Zhou, W., Liao, J., Zhang, W., Yuan, L., Hua, G., Yu, N.: E2style: Improve the efficiency and effectiveness of stylegan inversion. IEEE Transactions on Image Processing  \textbf{31},  3267--3280 (2022)

\bibitem{xie2022high}
Xie, J., Ouyang, H., Piao, J., Lei, C., Chen, Q.: High-fidelity 3d gan inversion by pseudo-multi-view optimization. arXiv preprint arXiv:2211.15662  (2022)

\bibitem{yang2021scene}
Yang, H., Zhang, Z., Yan, S., Huang, H., Ma, C., Zheng, Y., Bajaj, C., Huang, Q.: Scene synthesis via uncertainty-driven attribute synchronization. In: Proceedings of the IEEE/CVF International Conference on Computer Vision. pp. 5630--5640 (2021)

\bibitem{yang2015dense}
Yang, J., Li, H.: Dense, accurate optical flow estimation with piecewise parametric model. In: Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition. pp. 1019--1027 (2015)

\bibitem{yin20223d}
Yin, F., Zhang, Y., Wang, X., Wang, T., Li, X., Gong, Y., Fan, Y., Cun, X., Shan, Y., Oztireli, C., et~al.: 3d gan inversion with facial symmetry prior. arXiv preprint arXiv:2211.16927  (2022)

\bibitem{zhang2018unreasonable}
Zhang, R., Isola, P., Efros, A.A., Shechtman, E., Wang, O.: The unreasonable effectiveness of deep features as a perceptual metric. In: Proceedings of the IEEE conference on computer vision and pattern recognition. pp. 586--595 (2018)

\bibitem{zhu2020domain}
Zhu, J., Shen, Y., Zhao, D., Zhou, B.: In-domain gan inversion for real image editing. In: Computer Vision--ECCV 2020: 16th European Conference, Glasgow, UK, August 23--28, 2020, Proceedings, Part XVII 16. pp. 592--608. Springer (2020)

\bibitem{zhu2016generative}
Zhu, J.Y., Kr{\"a}henb{\"u}hl, P., Shechtman, E., Efros, A.A.: Generative visual manipulation on the natural image manifold. In: Computer Vision--ECCV 2016: 14th European Conference, Amsterdam, The Netherlands, October 11-14, 2016, Proceedings, Part V 14. pp. 597--613. Springer (2016)

\bibitem{zhu2017unpaired}
Zhu, J.Y., Park, T., Isola, P., Efros, A.A.: Unpaired image-to-image translation using cycle-consistent adversarial networks. In: Proceedings of the IEEE international conference on computer vision. pp. 2223--2232 (2017)

\end{thebibliography}


==> sec/experiment.tex <==
\section{Experiment}
\begin{comment}
\section{Experiment}
\begin{figure*}[t]  
\centering
\includegraphics[width=\textwidth]{figures/single_car/connect.png} 
%\vspace{-0.15in}
\caption{caption.}       %对图进行说明 
%\label{structure-1}  
%\vspace{-0.1in}
\end{figure*}
\end{comment}


\noindent\textbf{Datasets.}
%为了得到3D信息的真实值，我们使用GIRAFFE在数据集CompCars，Clevr，FFHQ，上预训练的模型生成我们的训练集和测试集。我们fllow GIRAAFE生成时的设定，在CompCars上我们预测公式8中提到的全部codes，在Clevr数据集上固定了物体的rotation和scale值，在FFHQ上固定了人脸的translation和scale值。同时为了测试我们的模型在in-the-wild数据上的性能，我们使用拍摄的真实场景下的车辆照片和CelebA-HQ的图像进行定性和定量的测试。
To obtain the true values of the 3D information in GIRAFFE for stable training performance, we use the pre-trained model of GIRAFFE on the CompCars~\cite{yang2015dense} dataset and Clevr~\cite{johnson2017clevr} dataset to generate training datasets. For testing datasets, we also use GIRAFFE to generate images for multi-car datasets denoted as \textit{G-CompCars} (CompCars is a single car image dataset) and use the original Clevr dataset for multi-geometry dataset (Clevr is a dataset that can be simulated to generate images of multiple geometries). We follow the codes setup in GIRAFFE. For CompCars, we use all the codes from Equation~\ref{codes}. For Clevr, we fixed the rotation, scale, and camera pose codes of the objects. For experiments on facial data, we utilized the FFHQ~\cite{karras2019style} dataset for training and the CelebA-HQ~\cite{karras2017progressive} dataset for testing.
\begin{comment}
\par To validate the performance of \sysname, we perform evaluations on G-CompCars and G-Clevr datasets for single-object and multi-object multifaceted editing tasks. We also compare the performance of 3D-GOI on an important sub-task, i.e., novel views synthesis of human faces, with the leading methods. Finally, we test 3D-GOI trained with \textit{G-dataset} on in-the-wild images, to reveal the limitations of GIRAFFE.
\end{comment}
\par \noindent\textbf{Baselines.}
%在神经反转编码器的对比实验中，我们对基于编码器的反转方法，以2D  GAN StyleGAN2为生成器的e4e,psp和以3D GAN EG3D为生成器的E3DGE和TriplaneNet与我们的神经反转编码器共同在GIRAFFE生成器上进行对比。同时我们也将我们的神经反转编码器在Style GAN2上，与同样基于Style GAN2的反转SOTA方法HyperStyle，HFGI和PTI 进行对比。
In the comparative experiments for our Neural Inversion Encoder, we benchmarked encoder-based inversion methods such as e4e~\cite{tov2021designing} and pSp~\cite{richardson2021encoding}, which use the 2D GAN StyleGAN2~\cite{karras2020analyzing} as the generator, and E3DGE~\cite{lan2023self} and TriplaneNet~\cite{bhattarai2023triplanenet} that employ the 3D GAN EG3D~\cite{chan2022efficient} as the generator, on the generator of GIRAFFE. Additionally, we compared our encoder on StyleGAN2 with SOTA inversion methods HyperStyle~\cite{alaluf2022hyperstyle} and HFGI~\cite{wang2022high} for StyleGAN2.

\par\noindent\textbf{Metrics.}
%我们使用MSE,LPIPS和SSIM来衡量图片的重建质量。
We use Mean Squared Error (MSE), perceptual similarity loss (LPIPS)~\cite{zhang2018unreasonable}, and identity similarity (ID) to measure the quality of image reconstruction.

\subsection{3D GAN Omni-Inversion}
\begin{table*}[!h]
%\setlength{\abovecaptionskip}{-0.1cm}
%\setlength{\belowcaptionskip}{0cm}
\centering
\setlength{\tabcolsep}{2.5mm}{
\begin{tabular}{c|c|c|c|c|c|c}  \hline
          \multirow{2}{*}{Method}    & \multicolumn{3}{c|}{ GIRAFFE for Generator}&\multicolumn{3}{c}{ StyleGAN2 for Generator} \\ \cline{2-7}
          &MSE $\downarrow$ & LPIPS $\downarrow$& ID$\uparrow$&MSE $\downarrow$ & LPIPS $\downarrow$&  ID$\uparrow$  \\    \hline
          e4e~\cite{tov2021designing}     &  0.031  & 0.306 &0.867  &  0.052  & 0.200 &0.502      \\ 
          pSp~\cite{richardson2021encoding}     &  0.031  & 0.301&0.877  &0.034& 0.172  &0.561    \\   
          HyperStyle~\cite{alaluf2022hyperstyle}& - & -   &  -        &   0.019  & 0.091  &0.766              \\ 
          HFGI~\cite{wang2022high}   &  - & - & - & 0.023& 0.124& 0.705    \\
       TriplaneNet~\cite{bhattarai2023triplanenet}      &  0.029  &0.296 &  0.870&-&-&-          \\ 
       E3DGE~\cite{lan2023self}     &0.031 & 0.299&0.881 & -&-  &- \\
        3D-GOI(Ours)   & \textbf{0.024}  &  \textbf{0.262} & \textbf{0.897} & \textbf{0.017} &\textbf{0.098}  &\textbf{0.769}\\   \hline
   %\caption{The results of FLOPs and the number of parameters}
\end{tabular}
}
%不同GAN inversion编码器在复杂场景下的重建结果
\caption{\footnotesize Reconstruction quality of different GAN inversion encoders using the generator of GIRAFFE and StyleGAN2. 
 $\downarrow$ indicates the lower the better and $\uparrow$ indicates the higher the better.}
\label{tab:compare_1}
\end{table*}


\subsection{Single-object Multifaceted Editing}
%如图我们展示了单个物体在两个数据集上的多元化编辑内容，(a),(b)，(c)是原图，经过编码器得到的粗略重建图和经过优化得到的精确图，可以看出像画面结构简单的clver数据集只使用编码器就可以得到相当精确的结果，而CompCars中的图像很难直接使用编码器预测出精准的codes，还需要循环优化算法进行优化才能得到精确的codes值,图4中的d-j和图5中的c-e是对这些codes的编辑结果，像我们在Section 3.4中说的，编辑物体朝前平移和放大物体的scale，可能会得到相似的图，由于篇幅限制我们部分图片内容像camera pose和clver的编辑shape等功能在supplement中展示。
%如图，与目前的先进的GAN inversion的模型相比，我们除了编辑物体和背景外，还可以对物体的仿射分量进行编辑更重要是可以编辑多物体
In Figure~\ref{fig:single_car} and Figure~\ref{fig:single_clver}, (a) depict the original images, the coarsely reconstructed images produced by the Neural Inversion Encoder, and the precisely reconstructed images obtained via round-robin optimization. As Figure~\ref{fig:single_clver} shows, the simple scene structure of the Clevr dataset allows us to achieve remarkably accurate results using only the encoder (Co-Recon). However, for car images in Figure~\ref{fig:single_car}, predicting precise codes using the encoder only becomes challenging, necessitating the employment of the round-robin optimization algorithm to refine the code values for precise reconstruction (Pre-Recon). Figure~\ref{fig:single_car} (b)-(h) and Figure~\ref{fig:single_clver} (b)-(d) show the editing results for different codes. As noted in Section~\ref{subsec:coarse}, moving an object forward and increasing its scale yield similar results. Due to space constraints, please refer to the Supplementary Material 4.1 for more results like camera pose and shape editing.
%\par As illustrated in Figure~\ref{fig:teaser}, compared with current state-of-the-art GAN inversion methods HyperStyle~\cite{alaluf2022hyperstyle}, our approach, in addition to editing the object and background, also permits editing of the affine information of the object.
%The model used on the G-Celeba-HQ dataset was trained on the G-FFHQ dataset.
%The former two tasks prove the innovative multi-object multifaceted edition ability of \sysname. The latter test proves \sysname\ has comparable performance with SOTA methods on the task face view change task while enabling rotation edition. %and current task of generating novel viewpoints via 3D GAN inversion for faces, 

\subsubsection{Multi-object Multifaceted  Editing}
\begin{comment}
\begin{figure}[t]  
%\setlength{\abovecaptionskip}{-0.1cm}
%\setlength{\belowcaptionskip}{-0.4cm}
\centering
\includegraphics[width=8.2cm]{figures/face/face.png} 
%\vspace{-0.15in}
\caption{\clc{Enlarge the fontsize and bold them}. Novel views synthesis for human faces using different GAN inversion methods.}       %对图进行说明 
\label{fig:face}  
%\vspace{-0.1in}
\end{figure}
\end{comment}
\begin{comment}
\begin{table}[t]
%\setlength{\abovecaptionskip}{-0.1cm}
%\setlength{\belowcaptionskip}{0cm}
\centering
\begin{tabular}{c|c|c|c|c}  \hline
          Method    & MSE $\downarrow$  & LPIPS $\downarrow$& ID$\uparrow$ & Speed(s)$\downarrow$  \\    \hline
            SG2     &  0.010  & 0.154 & 0.423 &  145.7       \\ 
      PTI      &  0.001  & 0.0478 &  0.839  &  54.93      \\   
       SPI     &  0.001  & 0.061&     0.957   &  550    \\ 
      3D-GOI   & 0.006  &  0.086 &   0.895 &30       \\   \hline
   %\caption{The results of FLOPs and the number of parameters}
\end{tabular}
\caption{ Reconstruction quality of different GAN inversion methods on \textit{G-CelebA-HQ}. $\downarrow$ means the lower the better and $\uparrow$ means the opposite.}
\label{tab:face}
\end{table}
\end{comment}


\begin{comment}
\begin{figure}[htbp]  
%\setlength{\abovecaptionskip}{-0.1cm}
%\setlength{\belowcaptionskip}{-0.4cm}
\centering
\includegraphics[width=1\textwidth]{figures/compare/compare_1.png}

%不同GAN Inversion方法的编码器在GIRAFFE生成器上的效果
\caption{\footnotesize Reconstruction results of different GAN inversion encoders using the generator of GIRAFFE.}       %对图进行说明 
\label{fig:compare_1}  
%\vspace{-0.1in}
\end{figure}
\end{comment}

%我们在多物体阶段使用的编码器都是在单物体场景训练的，我们发现对于物体的参数（obj_shape,obj_app,obj_s,obj_t,obj_r）预测的相对准确，而对于背景的预测差距较大，需要在优化阶段进行更细节的优化才可以得到准确的值。如图Fig6，7展示两辆车和多个Clevr物块的多元化编辑结果，车按照分别编辑然后一起编辑的顺序展示。从bin Fig6可以看出背景和左车的旋转角度预测差距很大，需要使用循环优化算法调整，我们将更多的多物体编辑图片放在补充材料中。
%In the multi-object editing, the encoders we utilized were all trained in single-object scenes. 
%We also train the encoders with single-object scenes for multi-object editing to reduce training costs, as explained in Section~\ref{sec:decomposition}.
We notice that the prediction for some object parameters ($obj\_shape$, $obj\_app$, $obj\_s$, $obj\_t$) are quite accurate. However, the prediction for the background codes deviates significantly. We speculate this is due to the significant differences in segmentation image input to the background encoder between multi-object scenes and single-object scenes. Therefore, background reconstruction requires further optimization. Figure~\ref{fig:two_cars} and Figure~\ref{fig:multi_clver} depict the multifaceted editing outcomes for two cars and multiple Clevr objects, respectively. The images show individual edits of two objects in the left and middle images and collective edits at the right images in Figure~\ref{fig:two_cars} (b-c) and (f-h). As demonstrated in Figure \ref{fig:two_cars}, the predictive discrepancy between the background and the rotation angle of the car on the left is considerable, requiring adjustments through the round-robin optimization algorithm. As illustrated in Figure~\ref{fig:teaser}, 2D/3D GAN inversion methods can not inverse multi-object scenes. More images pertaining to multi-object editing can be found in the Supplementary Material 4.2.
\subsection{Comparison Experiment of Neural Inversion Encoder}

\begin{figure} [t]
%\setlength{\abovecaptionskip}{-0.1cm}
%\setlength{\belowcaptionskip}{-0.7cm}
\begin{subfigure}{0.48\linewidth}
\centering
\includegraphics[width=0.87\textwidth]{figures/compare/compare_1.png}
    %\fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{\scriptsize Reconstruction results of different GAN inversion encoders using the generator of GIRAFFE.}
    \label{fig:compare_1}  
\end{subfigure}
\hfill
\begin{subfigure}{0.48\linewidth}
\centering
\includegraphics[width=1\textwidth]{figures/compare/compare_2.png}
    %\fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{\scriptsize Reconstruction results of different GAN inversion encoders using the generator of StyleGAN2.}
    \label{fig:compare_2}  
\end{subfigure}
\hfill
%图a是Giraffe中神经渲染的Block，是上采样的过程，图b是我们设计的与他相反的结构，是一个下采样过程。I是输入图片 Iv是图片的heatmap,HvWv，Mf是尺寸，w是要预测的code，w_f是w的维度
\caption{\scriptsize Reconstruction quality of different GAN inversion encoders.}
\label{fig:block}
\end{figure}

\begin{comment}
\begin{figure}[!h]  
%\setlength{\abovecaptionskip}{-0.1cm}
%\setlength{\belowcaptionskip}{-0.4cm}
\centering
\includegraphics[width=1\textwidth]{figures/compare/compare_1.png}

%不同GAN Inversion方法的编码器在GIRAFFE生成器上的效果
\caption{\footnotesize Reconstruction results of different GAN inversion encoders using the generator of GIRAFFE.}       %对图进行说明 

%\vspace{-0.1in}
\end{figure}

\begin{figure}[!h]  
%\setlength{\abovecaptionskip}{-0.1cm}
%\setlength{\belowcaptionskip}{-0.4cm}
\centering
\includegraphics[width=1\textwidth]{figures/compare/compare_2.png}

%不同GAN Inversion方法的编码器在GIRAFFE生成器上的效果
\caption{\footnotesize Reconstruction results of different GAN inversion encoders using the generator of StyleGAN2.}       %对图进行说明 
\label{fig:compare_2}  
%\vspace{-0.1in}
\end{figure}
\end{comment}

%为了进行公平的对比，消除生成器对反转图片生成质量的影响，我们将baseline方法中的编码器按照我们编码器NIE的训练方法连接GIRAFFE的生成器进行训练反转，与我们粗略估计得到的结果进行对比。同时我们也将我们的编码器连接StyleGAN2，与基于StyleGAN2的反转方法进行对比,以此证明我们设计NIE的高效性。
For fair comparison and to eliminate the impact of the generator on the quality of the inverted image generation, we trained the encoders from the baseline methods by connecting them to the GIRAFFE generator using our Neural Inversion Encoder training approach and compared them with our Neural Inversion Encoder. At the same time, we also connected our encoder to StyleGAN2 and compared it with inversion methods based on StyleGAN2, thereby demonstrating the efficiency of our encoder design.
%表1定量展示了我们编码器分别在GIRAFFE和StyleGAN2生成器上和baseline的比较结果，结果显示我们的NIB均优于目前的方法。
Table~\ref{tab:compare_1} quantitatively displays the comparison results on both the GIRAFFE and StyleGAN2 generators. The results show that our Neural Inversion Encoder consistently outperforms baseline methods.Figure~\ref{fig:compare_1} shows the performance comparison between our Neural Inversion Encoder and other baseline encoders using the GIRAFFE generator under the same training settings. Evidently, our method achieves the best results in both single-object and multi-object inversion reconstructions.
%图17展示了我们的方法使用StyleGAN2做编码器与同样基于StyleGAN2的baseline的对比结果，可以看见我们在头发，牙齿这些细节的反转上优于其他方法。
Figure~\ref{fig:compare_2} shows the performance comparison between our method and the baselines using StyleGAN2 as the generator. Our method clearly outperforms the baselines in the inversion of details such as hair and teeth.
%所以我们的神经反转编码器不论是定性和定量在不同的2D/3DGAN上均展现了卓越的反转能力
\par As such, we can conclude that our Neural Inversion Encoder performs excellent inversion on different 2D StyleGAN2 and 3D GIRAFFE, both qualitatively and quantitatively.
%图10展示了各个编码器，图10和table3的结果定性和定量展示了我们设计的NIE结构在对复杂场景图片反转
%Please refer to the qualitative results on the images in the Appendix~\ref{appendix_sec:comparison}.
\begin{comment}
\begin{table}[t]
%\setlength{\abovecaptionskip}{-0.1cm}
%\setlength{\belowcaptionskip}{0cm}
\centering
\begin{tabular}{c|c|c|c|c|c|c|c|c}  \hline
          \multirow{2}{*}{Method}    & \multicolumn{4}{c|}{ GIRAFFE for Generator}&\multicolumn{4}{c}{ StyleGAN2 for Generator} \\ \cline{2-9}
          &MSE $\downarrow$ & LPIPS $\downarrow$&MS-SSIM$\uparrow$& ID$\uparrow$&MSE $\downarrow$ & LPIPS $\downarrow$&MS-SSIM$\uparrow$ & ID$\uparrow$  \\    \hline
          e4e     &  0.031  & 0.306 & 0.471&0.867  &  0.052  & 0.200 & 0.721&0.502      \\ 
          pSp     &  0.031  & 0.301 &  0.523&0.877  &0.034& 0.172 & 0.760 &0.561    \\   
          HyperStyle& - & -  &-  &  -        &   0.019  & 0.091 & 0.849 &0.766              \\ 
          PTI     &  - & - & -& - & 0.015&  0.090& 0.92& 0.846    \\
       TriplaneNet     &  0.029  &0.296 &0.401 &  0.870&-&-&-&-          \\ 
       SPI     &0.031 & 0.299& 0.422&0.881 & -&- &- &- \\
        3D-GOI(Ours)   & 0.024  &  0.262 & 0.628 & 0.897& 0.017 &0.098 &0.886 &0.76\\   \hline
   %\caption{The results of FLOPs and the number of parameters}
\end{tabular}
%不同GAN inversion编码器在复杂场景下的重建结果
\caption{Reconstruction quality of different GAN inversion encoders using the generator of GIRAFFE.}
\label{tab:compare_1}
\end{table}
\end{comment}

\begin{comment}

\begin{figure}[t]  
%\setlength{\abovecaptionskip}{-0.1cm}
%\setlength{\belowcaptionskip}{-0.4cm}
\centering
\includegraphics[width=1\textwidth]{figures/order.png}

%不同GAN Inversion方法的编码器在GIRAFFE生成器上的效果
\caption{\footnotesize The figure of ablation study of the Round-robin Optimization algorithm.}       %对图进行说明 
\label{fig:order}  
%\vspace{-0.1in}
\end{figure}
    
\end{comment}
%我们同时测试人脸的新视角生成，注意这是目前3D GAN的主要任务，而这只是我们的一个很小的”功能“，图x展示了我们的方法与最新的3D inversion方法SPI以及一些可以生成新视角的先进2D GAN inversion方法PTI SG2的对比，表x中是我们的3D-GOI与这些方法重建质量的指标以及重建速度的对比。
\begin{comment}
\subsection{Novel views synthesis for human faces}
We also test the synthesis of novel views of human faces, which is the major ability of existing 3D GAN inversion methods but a sub-ability of \sysname. Figure~\ref{fig:face} shows that \sysname\ has similar performance with the latest 3D inversion method SPI~\cite{yin20223d} and some advanced 2D GANs that can generate novel views such as PTI~\cite{roich2022pivotal} and SG2~\cite{karras2020analyzing}. Table~\ref{tab:face} summarizes the metric values of the reconstruction quality and the speed, showing that \sysname\ has a clear advantage in speed.
\end{comment}


 




%由于GIRAFFE的生成质量不高，如果想迁移到真实的in the wild的分布，我们需要在优化时也把生成器加入训练，但结果如图x所示,可以看出来我们还是无法完美还原原图尤其是背景，这说明GIRAFFE的生成器无法生成真实的图像分布，我们对比发现其参数量是生成同样大小图像的stylegan2的1/40，如果修改GIRAFFE结构，增加网络参数使其生成接近真实图片的分布，那么我们3D-GOI的就可以反转真实图片
\begin{comment}
\subsection{In-the-wild images}
Due to the significant difference between the data distribution generated by GIRAFFE and that of in-the-wild images, we add the generator parameters in the optimization process. As shown in Figure \ref{fig:wild}, 3D-GOI cannot perfectly reconstruct the original image, especially the background. %This suggests that the GIRAFFE generator cannot generate a realistic image. 
We compared and found that the number of parameters of the generator in GIRAFFE is $1/40$ of that of StyleGAN2~\cite{karras2020analyzing}.\textcolor{red}{We think if we modify the structure of GIRAFFE to enable it to generate a distribution closer to real images, then \sysname\ can successfully edit real images.}
\end{comment}
\subsection{Ablation Study}

\begin{comment}
\begin{table}[t]
\centering
  \begin{tabular}{c|c|c|c}  \hline
          Method    & MSE $\downarrow$  & LPIPS$\downarrow$ & ID $\uparrow$\\    \hline
        
        w/o NIB  & 0.023 & 0.288  &      0.856        \\ 
        w/o MLP &   0.015 &    0.183  &    0.878      \\ 
         3D-GOI    &  \textbf{0.010} & \textbf{0.141} &  \textbf{0.906}         \\ \hline
\end{tabular}
       

  \caption{\footnotesize Ablation Study of the Neural Inversion Encoder.}   
 \label{tab:NIE}

\end{table}


\begin{table}[t]
\begin{tabular}{c|c|c|c}  \hline
          Method    & MSE $\downarrow$  & LPIPS $\downarrow$& ID$\uparrow$   \\    \hline
        Order1     &  0.016  & 0.184 & 0.923       \\ 
       Order2      &  0.019  & 0.229 &  0.913      \\   
        Order3      &  0.019  & 0.221&     0.911     \\ 
      3D-GOI   & \textbf{0.008}  & \textbf{ 0.128} &   \textbf{0.938}       \\   \hline
   %\caption{The results of FLOPs and the number of parameters}
\end{tabular}

 \caption{\footnotesize The quantitative metrics of  ablation study of the Round-robin Optimization algorithm.}
\label{tab:order}

\end{table}
\end{comment}
\begin{table}[t]
%\setlength{\abovecaptionskip}{-0.1cm}
%\setlength{\belowcaptionskip}{0cm}
\centering
\begin{floatrow}
\capbtabbox{
  \begin{tabular}{c|c|c|c}  \hline
          Method    & MSE $\downarrow$  & LPIPS$\downarrow$ & ID $\uparrow$\\    \hline
        
        w/o NIB  & 0.023 & 0.288  &      0.856        \\ 
        w/o MLP &   0.015 &    0.183  &    0.878      \\ 
         3D-GOI    &  \textbf{0.010} & \textbf{0.141} &  \textbf{0.906}         \\ \hline
\end{tabular}
       
}{
  \caption{\footnotesize Ablation Study of the Neural Inversion Encoder.}   
 \label{tab:NIE}
}
\capbtabbox{
\begin{tabular}{c|c|c|c}  \hline
          Method    & MSE $\downarrow$  & LPIPS $\downarrow$& ID$\uparrow$   \\    \hline
        Order1     &  0.016  & 0.184 & 0.923       \\ 
       Order2      &  0.019  & 0.229 &  0.913      \\   
        Order3      &  0.019  & 0.221&     0.911     \\ 
      3D-GOI   & \textbf{0.008}  & \textbf{ 0.128} &   \textbf{0.938}       \\   \hline
   %\caption{The results of FLOPs and the number of parameters}
\end{tabular}
}{
 \caption{\footnotesize The quantitative metrics of  ablation study of the Round-robin Optimization algorithm.}
\label{tab:order}
}
\end{floatrow}
\end{table}


\begin{figure}[t]  
%\setlength{\abovecaptionskip}{-0.1cm}
%\setlength{\belowcaptionskip}{-0.4cm}
\centering
\includegraphics[width=1\textwidth]{figures/order.png}

%不同GAN Inversion方法的编码器在GIRAFFE生成器上的效果
\caption{\footnotesize The figure of ablation study of the round-robin Optimization algorithm.}       %对图进行说明 
\label{fig:order}  
%\vspace{-0.1in}
\end{figure}
%我们对比了加入神经反转Block和多层MLP对编码器性能的影响，以及循环神经算法中是否可以合并多个变量进一个编码器中,更多的对比实验我们放到补充材料中
We conducted ablation experiments separately for the proposed Neural Inversion Encoder and the Round-robin Optimization algorithm.

\par Table~\ref{tab:NIE} displays the average ablation results of the Neural Inversion Encoder on various attribute codes, where NIB refers to Neural Inversion Block (the second part of the encoder) and MLP is the final part of the encoder. The results clearly show that our encoder structure is extremely effective and can predict code values more accurately. Please find the complete results in the  Supplementary Material 4.4.
\par For the Round-robin optimization algorithm, we compared it with three fixed optimization order algorithms on both single-object and multi-object scenarios. The three fixed sequences are as follows:
\par $Order1: bg\_shape, bg\_app, \{obj\_r_i,obj\_t_i, obj\_s_i\}_{i=1}^{N}, \\ \{obj\_shape_i, obj\_app_i\}_{i=1}^{N}, camera\_pose$
\par $Order2: \{obj\_r_i,obj\_t_i, obj\_s_i\}_{i=1}^{N}, \{obj\_shape_i, \\ obj\_app_i\}_{i=1}^{N}, bg\_shape, bg\_app, camera\_pose$
\par $Order3: camera\_pose, \{obj\_shape_i, obj\_app_i\}_{i=1}^{N}, \\ \{obj\_r_i, obj\_t_i, obj\_s_i\}_{i=1}^{N}, bg\_shape, bg\_app$ 
\par $\{\}_{i=1}^{N}$ indicates that the elements inside $\{\}$ are arranged in sequence from 1 to N. There are many possible sequence combinations, and here we chose \textbf{the three with the best results} for demonstration. Table~\ref{tab:order} and Figure~\ref{fig:order} are  the quantitative and  qualitative comparison of the four methods. As shown, our method achieves the best results on all metrics, demonstrating the effectiveness of our Round-robin optimization algorithm. As mentioned in  \ref{sec:4.4}, optimizing features like the image background first can enhance the optimization results. Hence, Order1 performs much better than Order2 and Order3. 
%\par More comparative and ablation experiments can be found in the Supplementary Material.



\begin{comment}
\begin{table}[t]
\setlength{\abovecaptionskip}{-0.1cm}
\setlength{\belowcaptionskip}{-0.05cm}
\centering
\begin{tabular}{c|c|c|c}  \hline
          Method    & MSE $\downarrow$  & LPIPS$\downarrow$ & ID $\uparrow$\\    \hline
        
       3D-GOI w/o NIB  & 0.023 & 0.288  &      0.856        \\ 
       3D-GOI w/o MLP &   0.015 &    0.183  &    0.878      \\ 
         3D-GOI    &  0.010 & 0.141 &  0.893         \\ \hline
           
\end{tabular}
\caption{Ablation Study of the Neural Inversion Encoder.}
\label{tab:inversion_methods}
\end{table}
\end{comment}



==> sec/method.tex <==
%\subsection{Related Models}
%预备知识： Nerf是最近很流行的3D重建任务的方法，它使用神经辐射场建模场景，可以将空间中任意一个视角方向和空间坐标的高维位置编码映射成颜色和不透明度，并用体渲染公式合成对应视角下的图片。神经辐射场的映射函数用f表示，\theta是其参数，公式一中r是位置编码函数，用于添加高维信息到x和d上，得到的维数为lx和ld的输出。公式2描述的是在给定相机射线r(t) = o + td在远近区间内预测的颜色的体渲染公式，T(t)表示沿射线从tn到t的累积透射率。生成式神经辐射场，Graf在Nerf的基础上输入中额外添加物体形状和颜色的潜在分量，不仅可以控制生成物体的外观而且可以控制生成不同相机视角下的图像，GIRAFFE在此的基础上推广到多物体场景，他认为图像场景是由背景和多个物体通过仿射变换结合起来的，每一个物体可以通过放缩，平移和旋转变换到图像中的特定位置。GIRAFFE合并多物体时并没有使用颜色的加权而是使用每个物体的特征场相加，特征场是GIRAFFE在公式x的基础上将R3的颜色值转换为高维的特征场，于是GIRAFFE将渲染阶段分为两部分，第一部分使用特征代替颜色值完成体渲染，这样得到的是一个特征图谱，所以第二阶段神经渲染将特征图生成图片。
%问题定义：我们的任务是给将输入图像反转成GIRAFFE生成器生成这张图时的所有参数，从而可以对图片进行多元化灵活的编辑。和2D的反转任务一样，我们先进行输入图片的重建。我们用G表示GIRAFFE的生成器，I表示输入的图片，W表示GIRAFFE生成时所需要的参数。w由物体形状obj_s,物体外观obj_a，物体放缩分量obj_s,物体平移分量obj_t，物体旋转分量obj_r，背景形状分量bg_s,背景外观分量bg_a以及相机角度量cam_p，由于有多个物体，所以我们将w表示为。那么我们的inversion任务的重建部分就可以表示为.我们的任务是极具挑战性的，目前GAN反转的方法通常只是预测一个潜在分量，即便是3D GAN也只是多预测一个相机位姿的矩阵（基于style gan的多个style分量是由一个初始量生成的，他们之间是相关的，往往只需要一个编码器就可以预测全部量），而我们需要预测5n+3个独立的分量，n是物体的个数。
%3.1中4567公式介绍了GIRAFFE首先将各个物体的各个分量输出成一个特征场，再将各个物体特征场合成后再通过体渲染和神经渲染得到最后的图像，所以我们要想反向独立的得到每个物体和背景的各个分量，最直接的思考是先分离他们。如果要对基于数学的角度分解原来的叠加的特征场是非常困难的，即便设计一个反向网络可以得到精确的特征叠加场，由于我们不知道每个物体的加权系数，我们也无法对其分解。以图x为例子，从渲染公式角度来看，我们在A区域可以看到A车而看不到B车，就说明A车在对应位置上特征的权重可能远大于B车，于是我们打印了GIRAFFE在特征场合成时不同物体的不透明度，我们发现，A物体只在区域A的不透明度值很高，而在其余地方很低（趋于0），同理B车在区域B不透明度很高，而其余地方很低（趋于0），背景是在全图区域内都有不透明度的值，没有明显的极高极低值。由于A车和B车在背景区域的不透明度值很低（趋于0），所以我们认为背景区域部分的特征场只由背景的特征组成，由于A车在A区域的不透明度远大于背景和b车，所以我们可以近似认为区域A的特征场只由A车的特征表达，同样区域B的特征场只有B车的特征表达，那么这样我们就可以反向根据各个区域的色素值估计出各个物体（A，B车和背景）的特征值最后估计出他们的潜在分量，所以我们采用图像分割方法就可以近似分离原来的特征场。
%反渲染编码器的设计与训练，我们使用编码器来直接对code进行一个粗略估计，与一般基于编码器的inversion方法不同，我们的潜在分量无法只用一个编码器全部预测完，所以我们为每一个分量都分配一个编码器，每个编码器的结构是相似的。以下说明我们的设计思路，我们根据GIRAFFE的神经渲染器和提渲染器反向设计反转网络。我们的反转网络分为三个部分，第一个部分是使用E4E网络的骨架结构提取图片的特征，第二部分使用提取特征和输入的图片通过神经反转区块得到一维的特征向量,最后使用不同的MLP结构得到对应的维度的潜在分量。神经反转区块我们通过将图片使用CNN逐层下采样然后使用跳跃连接逐层连接特图谱后得到尺寸是一维的特征，如图我们的结构和GIRAFFE的神经渲染结构差不多是相反的。最后一层使用MLP结构是因为我们考虑到潜在分量是在GIRAFFE的MLP层前就加入的，所以逆向的计算的时候我们希望可以通过MLP还原这些分量，而且每个潜在分量的维度（用词？）是不一样的，我们需要一种灵活可以改变输出维数的网络结构，显然MLP是很好的选择。像第一章说的，多个潜在分量同时训练模型基本不会收敛，所以我们使用GIRAFFE生成的数据集训练，这样我们可以保存各个潜在分量的真实值，每次只训练一个潜在分量的编码器，保留其他潜在分量是真实值。在训练物体的时我们使用生成图片和原图的mse损失，感知损失，以及id损失，这个和大多数的2D GAN训练是一致的，在训练仿射分量（放缩量s,平移量t,旋转量r）我们发现不同的组合值会生成非常相似的图片（比如车辆向前平移和整体放大在视觉上只有细微差别），也就是说不同的图片的仿射值并不是唯一解，为了加速训练以及提高重建效果，我们在loss中加入预测的str值和真实值的mse的损失，迫使编码器直接预测真实值。
%循环神经优化算法，上一步编码器预测出一个粗略的结果，我们在此的基础上优化各个codes值，我们在实验中发现只使用一个优化器同时优化8个潜在分量容易导致不稳定的优化进程，所以我们类似的像上一步使用多个优化器分别优化各个变量。我们发现优化顺序对整个优化结果至关重要，不同的编码器预测的code与真实值的误差大小不一样，不同code改变对图像的影响也不一样（比如控制背景生成的code改变会对图片整体像素有较大影响），所以我们提出了一个自动化的循环优化算法，可以根据每轮重建的图像对各个code进行优化排序自动化进行多轮优化。我们的排序算法思路是对各个变量进行多次微小扰动，计算扰动后前后重建的图像间与原图像之间的损失，如果损失变大，说明当前code值相对准确，优化顺序排后，如果变小，说明对于当前code值不准确需要优先优化，对于多个都需要先优化的值，我们使用loss变化量和扰动量的偏导来计算他们之间的优先级。旋转角度r来说，我们发现添加深度损失对其可以加速其优化，不在encoder中是因为加入会拖慢训练速度而且结果并没有明显的影响。对于单个物体，按照r,物体形状颜色，s,t，背景颜色和形状进行优化，前一步对物体旋转角度预测往往有较大的误差，所以在实际中我们会对差距较大的图片的旋转角度进行采样，选取loss。而对于多物体的图片，由于我们是使用分割的方法
% Applied to in-the-wild pictures :在之前的训练和测试中，为了获得各个code的真实值，我们使用的是GIRAFFE生成的数据集，我们尝试直接将模型使用在真实拍摄的照片上，发现无论怎么优化都无法重建原图片，这是由于GIRAFFE生成的数据分布和in-the-wild pictures分布有着很大的差别，所以为了推广到in-the-wild pictures上，我们还需要调整GIRAFFE生成器的参数。
%deepl：Nerf is a reconstruction task that, given a viewpoint and coordinates, returns the colour and opacity of that point and then synthesises the colour on the ray according to the body rendering formula.Nerf GAN, like Graf, adds additional potential components of object shape and colour to the input on the basis of Nerf to control the shape of the object, and GIRAFFE extends this to multi-object scenes. In the rendering stage GIRAFFE considers that the superposition of colours at the same point in space for multiple objects is not a simple pigment weighting, so it considers the use of a feature field superposition instead of a colour superposition, so GIRAFFE divides the rendering stage into two parts. The first part uses features instead of colour values to complete the body rendering, so that a feature map is obtained, so the second stage neural rendering generates the feature map into a picture
\begin{figure*}[t]
%\setlength{\abovecaptionskip}{-0.1cm}
%\setlength{\belowcaptionskip}{-0.5cm}
\begin{subfigure}{0.3\linewidth}
\includegraphics[width=0.8\textwidth]{figures/2dgan_2.png}
    %\fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{2D GANs}
    % \label{fig:short-a}
\end{subfigure}
\hfill
\begin{subfigure}{0.3\linewidth}
\includegraphics[width=0.8\textwidth]{figures/3dgan_2.png}
    %\fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{3D GANs}
    % \label{fig:short-a}
\end{subfigure}
\hfill
\begin{subfigure}{0.3\linewidth}
\includegraphics[width=0.8\textwidth]{figures/giraffe_2.png}
    %\fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{GIRAFFE}
    % \label{fig:short-a}
\end{subfigure}

%图a是普通的2D GAN和GAN Inversion方法，一个潜在编码对应一张图片，图b是普通的3D GAN和GAN Inversion方法,一般多一个相机位姿的code，这两种方法都只能生成和反转单物体，图三是GIRAFFE，它可以生成多物体复杂的场景，每个物体由颜色形状放缩平移和旋转量控制，背景由颜色形状控制，同样由c控制相机位姿，所以一般由5n+3个code，远超一般GAN的code数量，所以对其进行反转是一项非常有挑战的工作。
 \caption{ \scriptsize  Figure (a) represents the typical 2D GANs and 2D GAN Inversion methods, where one latent encoding corresponds to one image. Figure (b) represents the typical 3D GANs and 3D GAN Inversion methods, which usually have an additional camera pose code c. Both of these methods can only generate and invert single objects. Figure (c) represents GIRAFFE, which can generate complex multi-object scenes. Each object is controlled by appearance, shape, scale, translation, and rotation, while the background is controlled by appearance and shape. Similarly, c controls the camera pose, so there are generally (5n+3) codes, far more than the number of codes in a typical GAN. Therefore, inverting it is a very challenging task.'bg' means background and 'obj' means object.}
 \vspace{-0.3cm}
\label{fig:gans}
\end{figure*}

\section{\sysname}
\vspace{-10pt}
In this section, we present the problem definition of \sysname\ and our three-step inversion method: scene decomposition, coarse estimation, and precise optimization, as depicted in Figure~\ref{fig:overall}.
\subsection{Problem Definition}
%我们要解决的问题与一般的3D GAN inversion的定义类似，区别在我们需要反转的变量远超过2个。我们将GIRAFFE生成器中的所需的变量分为三类
The problem we target is similar to the general definition of  GAN inversion, with the difference being that we need to invert many more codes than existing methods(1 or 2)  as shown in Figure~\ref{fig:gans}. The parameter $w$ in GIRAFFE, which controls the generation of images, can be divided into three categories: object attributes, background attributes, and pose attributes. We use the prefix \textit{obj} to denote object attributes, \textit{bg} for background attributes, and \textit{$camera\_pose$} for pose attributes. As such, $w$ can be denoted as follows:
\begin{equation}
    \begin{aligned}
        W = \{ obj\_shape_i, obj\_app_i , obj\_s_i, 
        obj\_t_i , obj\_r_i , \\ bg\_shape, bg\_app ,cam\_pose \} \quad  i = 1,...,n  ,
    \end{aligned}
\label{codes}
\end{equation}
where $obj\_shape$ is the object shape latent code, $obj\_app$ is the object appearance latent code, $obj\_s$ is the object scale code, $obj\_t$ is the object translation code, $obj\_r$ is the object rotation code, $bg\_shape$ is the background shape latent code, $bg\_app$ is the background appearance latent code and $cam\_pose$ is the camera pose matrix. $n$ denotes the $n$ objects. Then, the reconstruction part of the inversion task can be expressed as:
\begin{equation}
    W^{*} = arg \mathop{\min}_{W} \mathcal{L}(G(W,\theta),I) ,
\end{equation}
where $G$ denotes the generator, $\theta$ denotes the parameters of the generator, $I$ is the input image, and $\mathcal{L}$ is the loss function measuring the difference between the generated and input image.
%where $G$ represents the GIRAFFE generator, $I$ stands for the input image, $\mathcal{L}$ represents the loss function that can measure the difference between the input image $I$ and the reconstructed image $G(w,\theta)$.
According to Equation\ref{codes}, we need to invert a total of $(5n+3)$ codes. Then, we are able to replace or interpolate any inverted code(s) to achieve multifaceted editing of multiple objects.


\begin{figure*}[t]
%\setlength{\abovecaptionskip}{-0.1cm}
%\setlength{\belowcaptionskip}{-0.5cm}
\begin{subfigure}{0.24\linewidth}
\centering
\includegraphics[width=0.6\textwidth]{figures/image.png}
    %\fbox{\rule{0pt}{2in} \rule{.6\linewidth}{0pt}}
    \caption{Input}
    % \label{fig:short-a}
\end{subfigure}
\hfill
\begin{subfigure}{0.24\linewidth}
\centering
\includegraphics[width=0.6\textwidth]{figures/carA.png}
    %\fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Car A}
    % \label{fig:short-a}
\end{subfigure}
\hfill
\begin{subfigure}{0.24\linewidth}
\centering
\includegraphics[width=0.6\textwidth]{figures/carB.png}
    %\fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Car B}
    % \label{fig:short-a}
\end{subfigure}
\hfill
\begin{subfigure}{0.24\linewidth}
\centering
\includegraphics[width=0.6\textwidth]{figures/background.png}
    %\fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Background}
    % \label{fig:short-a}
\end{subfigure}


%图a是输入图片，图B是A车特征权重图，颜色越红的表示A车不透明度越高，越蓝表示越低，同样的图C是B车的特征权重图，图d是背景的特征权重图，将这几幅图结合起来可以看到A车区域近似就只有A的特征表达同理B车区域只有B车特征表达，可视的背景区域只有背景的特征表达。
\caption{\scriptsize Scene decomposition. (a) is the input image. (b) is the feature weight map of car A, where the redder regions indicate a higher opacity for car A and the bluer regions indicate lower opacity. Similarly, (c) is the feature weight map of car B, and (d) represents the feature weight map of the background. By integrating these maps, it becomes apparent that the region corresponding to car A predominantly consists of the feature representation of car A and likewise for car B. And the visible area of the background solely contains the feature representation of the background.}
\vspace{-0.3cm}
\label{fig:decomposition}
\end{figure*}

\subsection{Scene Decomposition}
\label{sec:decomposition}
\vspace{-10pt}
%我们人观察图像，可以很简单的分辨每个物体以及其的一些特征（颜色形状），但是这对于机器来说是十分复杂的，涉及目标检测，目标分割，分类等等，
%这里要说明分割场景是为了给多物体场景做准备
%正如前面章节所说，GIARFFE生成器与一般的GAN生成器不同，在生成图片时有大量的codes参与，并不是一个code控制图像所有部分生成，所以我们很难与一般的GAN Inversion方法一样，只使用一个编码器或者优化器转化出所有的codes.我们人观察图像，可以很简单的分辨每个物体以及其的一些特征（颜色形状），但是这对于机器来说是十分复杂的，需要大量高精度的标注样本，才能让机器理解图片中什么位置表达了什么的code。我们希望先粗略的将不同的codes分离出来，从而简化问题。根据公式4和5，图像中的物体在什么位置显示什么样的形状颜色，是物体经过了仿射变换以及zs和za控制表达的，由公式6特征合成公式以及公式7渲染公式可知，不透明度控制特征表达的系数，所以渲染图像是物体的地方，其对应的特征场的不透明度就很高，是背景的地方，其对应的特征场的不透明度会很高。所以，我们可以只使用简单分割预训练将图片分割成不同的物体和背景，这样就可以像公式10中将code分成八大类（cam_pose需要整个渲染图像的信息才能得到）。
%
As mentioned in previous sections, the GIRAFFE generator differs from typical GAN generators in that a large number of codes are involved in generating images, and not a single code controls the generation of all parts of the image. Therefore, it is challenging to transform all codes using just one encoder or optimizer as in typical GAN Inversion methods. A human can easily distinguish each object and some of its features (appearance, shape) from an image, but a machine algorithm requires a large number of high-precision annotated samples to understand what code is expressed at what position in the image.
\begin{comment}
Therefore, we first simplify the problem by separating the different codes on a coarse granularity. According to Eq. (4) and (5), what kind of shape and color an object in the image shows at what position is controlled by the affine transformation of the object and by $\bm{z_s}$ and $\bm{z_a}$. According to Eq. (6), the feature synthesis formula, and Eq. (7), the rendering formula, the opacity controls the coefficient of feature expression. Therefore, when the rendered image is an object, the opacity of the corresponding feature field is very high, and for the background, the opacity of the corresponding feature field is very low.

Thus, we can use pre-trained segmentation to divide the image into individual objects and the background, allowing us to divide the code into 8 major categories defined in Eq. (10). Note that obtaining $cam\_pose$ requires information from the entire rendered image.
%我们从定性的角度证明这简单的分割是可行的，我们打印了GIRAFFE在特征场合成时不同物体在各个位置上的不透明度，结果如图3所示，A车在其区域内不透明度值很高而在其他位置几乎为0，B车同理，背景则是在整个场景中都有不规律的透明度分布。通过特征场合成公式6，我们可以近似认为在A/B车和背景只在其可视的区域内有特征场的表达，所以就可以用简单的分割方法将每个特征场分离。
We demonstrate the feasibility of the segmentation method from a qualitative perspective. Figure~\ref{car} illustrates the opacity of different objects at various locations during the process of feature field synthesis in GIRAFFE. For instance, car A exhibits a high opacity value within its own area and near-zero opacity elsewhere - a similar pattern is seen with car B. The background, however, presents a non-uniform opacity distribution across the entire scene. 
Drawing upon the feature field synthesis in Eq.~\ref{giraffe-3}, we can  consider that both car A and car B and the background mainly manifest their feature fields within their visible areas. Hence, we apply a straightforward segmentation method to separate each object's feature field. The feature field is obtained from the various object codes using Eq.~\ref{giraffe-2}. In this way, we separate the codes of different objects and the background on a coarse granularity to simplify the problem.
\end{comment}
%一个直观的思想是：在多物体图片中，一个物体的attrubute codes的表达会映射到图片中相应物体的位置上，例如平移旋转code控制物体在场景中相对位置，放缩和shapecode控制着物体的轮廓形状，颜色code控制物体所在位置颜色的表达。使用分割得到的图像包含上述三种信息，我们可以通过其反转得到对应物体的五个attribute codes。
\par A straightforward idea is that in images with multiple objects, the attribute codes of an object will map to the corresponding position of the object in the image. For example, translation ($obj\_t$) and rotation ($obj\_r$) codes control the relative position of an object in the scene, scaling ($obj\_s$) and shape ($obj\_shape$) codes determine the contour and shape of the object, and appearance ($obj\_app$) codes control the appearance representation at the position of the object. The image obtained from segmentation precisely encompasses these three types of information, allowing us to invert it and obtain the five attribute codes for the corresponding object. Similarly, for the codes ($bg\_app,bg\_shape$) that generate the background, we can invert them using the segmented image of the background. Note that obtaining $cam\_pose$ requires information from the entire rendered image.

\par We can qualitatively validate this idea. In Equation~\ref{equ:map}, we can see that an object's five attribute codes are mapped to the object's feature field and volume density through $h_{\theta}$. As inferred from Equation~\ref{equ:composition}, the scene's feature field is synthesized by weighting the feature fields of each object by density. Therefore, the reason we see an object appear at its position in the scene is due to its feature field having a high-density weight at the corresponding location. Figure~\ref{fig:decomposition} displays the density of different objects at different positions during GIRAFFE's feature field composition process. The redder the color, the higher the density, while the bluer the color, the lower the density. As we discussed, car A exhibits a high-density value within its own area and near-zero density elsewhere - a similar pattern is seen with car B. The background, however, presents a non-uniform density distribution across the entire scene. we can consider that both car A and car B and the background mainly manifest their feature fields within their visible areas. Hence, we apply a straightforward segmentation method to separate each object's feature field and get the codes. 

%将每个物体分割还有一个重要的好处，这样使得我们后续设计的编码器更加关注每个输入的物体或是背景，我们就可以在单物体场景上训练编码器然后直接推广到多物体的场景下（在多物体场景下训练涉及更多codes，成本太高）
\par Segmenting each object also has an important advantage: it allows our encoder to pay more attention to each input object or background. As such, we can train the encoder on single-object scenes and then generalize it to multi-object scenes instead of directly training in multi-object scenes that involve more codes, to reduce computation cost.

\begin{figure} [t]
%\setlength{\abovecaptionskip}{-0.1cm}
%\setlength{\belowcaptionskip}{-0.7cm}
\begin{subfigure}{0.45\linewidth}
\centering
\includegraphics[width=0.8\textwidth]{figures/neuralrender.png}
    %\fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Neural Rendering Block}
    % \label{fig:short-a}
\end{subfigure}
\hfill
\begin{subfigure}{0.45\linewidth}
\centering
\includegraphics[width=0.8\textwidth]{figures/in-neuralrender.png}
    %\fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Neural Inversion Encoder}
    % \label{fig:short-a}
\end{subfigure}
\hfill


%图a是Giraffe中神经渲染的Block，是上采样的过程，图b是我们设计的与他相反的结构，是一个下采样过程。I是输入图片 Iv是图片的heatmap,HvWv，Mf是尺寸，w是要预测的code，w_f是w的维度
\caption{\scriptsize The design of Neural Inversion Encoder. (a) represents the Neural Rendering Block in GIRAFFE~\cite{niemeyer2021giraffe}, which is an upsampling process to generate image $\hat{I}$. In contrast, (b) illustrates the Neural Inversion Encoder that opposes it, which is a downsampling process. $I$ is the input image, $H,W$ are image height and width. $I_v$ denotes the heatmap of the image, $H_v,W_v$ and $M_f$ are the dimensions of $I_v$, $w$ is the code to be predicted, and $w_f$ is the dimension of $w$. Up means upsampling and Down means downsampling.}
\vspace{-0.3cm}
\label{fig:block}
\end{figure}
\subsection{Coarse Estimation}\label{subsec:coarse}
\vspace{-0.3cm}
%我们在上一步分割后的基础上，使用编码器来粗略估计各个codes.与一般基于编码器的方法不同，只使用一个编码器很难预测出所有的codes,同时也为了方便训练，我们为每一个code分配一个编码器，让每一个编码器只专注于一个code的预测，所以总共需要8个编码器。
The previous segmentation step roughly disentangles the codes. Unlike typical encoder-based methods, it's difficult to predict all codes using just one encoder. Therefore, we assign an encoder to each code, allowing each encoder to focus solely on predicting one code.  Hence, we need a total of eight encoders. As shown in Figure~\ref{fig:overall}, we input the object segmentation for the object attribute codes ($obj\_shape, obj\_app, obj\_s, 
        obj\_t, obj\_r$), the background segmentation for the background attribute codes ($bg\_shape, bg\_app$), and the original image for pose attribute code ($cam\_pose$). Different objects share the same encoder for the same attribute code. 
\par We allocate an encoder called Neural Inversion Encoder with a similar structure to each code. 
Neural Inversion Encoder consists of three parts as Figure~\ref{fig:block}(b) shows. The first part employs a standard feature pyramid over a ResNet~\cite{he2016deep} backbone like in pSp~\cite{richardson2021encoding} to extract the image features. The second part, in which we designed a structure opposite to GIRAFFE's Neural rendering Block based on its architecture as Figure~\ref{fig:block}(a) shows, downsamples the images layer by layer using a Convolutional Neural Network (CNN) and then uses skip connections~\cite{he2016deep} to combine the layers, yielding a one-dimensional feature. The third layer employs an MLP structure to acquire the corresponding dimension of different codes. Please refer to the Supplementary Materials 3.1 for the detailed structure of our Neural Inversion Encoder.

 
\par Training multiple encoders simultaneously is difficult to converge due to the large number of training parameters. Hence, we use the dataset generated by GIRAFFE for training to retain the true values of each code and train an encoder for one code at a time, to keep the other codes at their true values. Such a strategy greatly ensures smooth training.  

During encoder training, we use the Mean Squared Error (MSE) loss, perceptual loss (LPIPS)~\cite{zhang2018unreasonable}, and identity loss (ID)~\cite{he2020momentum} between the reconstructed image and the original image, to be consistent with most 2D and 3D GAN inversion training methodologies. When training the affine codes (scale $s$, translation $t$, rotation $r$), we find that different combinations of values produce very similar images, e.g., moving an object forward and increasing its scale yield similar results. However, the encoder can only predict one value at a time, hence we add the MSE loss of the predicted $s$,$t$,$r$ values, and their true values, to compel the encoder to predict the true value.

\begin{equation}
    \mathcal{L}_{enc} = \lambda_1 L_2 + \lambda_2 L_{lpips} + \lambda_3 L_{id} \label{loss_enc} ,  
\end{equation}
where $\lambda_i,i=1,2,3$ represent the ratio coefficient between various losses. When training $obj\_s,obj\_t,obj\_r$ code, the $L_2$ loss includes the MSE loss between the real values of $obj\_s,obj\_t,obj\_r$ and their predicted values.
%deepl:The recurrent neural optimization algorithm, with multiple encoders predicting a rough result in the previous step. We build on this to optimise the individual latent variable values. We found in our experiments that using only one optimiser for the eight latent components tends to lead to an unstable optimisation process, so we similarly use multiple optimisers, with one optimiser for object shape and colour and one optimiser for each of the other components. For the rotation angle r, we found that adding a depth loss to it accelerated its optimisation, not in the encoder because adding it slowed down the training and did not have a significant impact on the results. For a single object, the optimisation is done according to r, object shape colour, s,t, background colour and shape, the previous step often has a large error in predicting the rotation angle of the object, so in practice we sample the rotation angle of images with large gaps and select the loss.
\begin{comment}
\begin{algorithm}[t]
%\SetAlgoNoLine
\caption{Round-robin Optimization}
\label{alg:one}
\KwData{all codes $w \in W$ predicted by encoders, fixed GIRAFFE generator $G$, input image $I$;}
Initialize $lr\_w = 10^{-3} ,w\in W$ \;
\While{any $lr\_w > 10^{-5}$}{
     \ForEach{ $w \in W$}{
            Sample $\delta w$\;
            Compute $\delta \mathcal{L}(w)$ using Eq.8;
     }
     Compute $rank\_list$ using Eq.9;
     \ForEach{ $w \in rank\_list$ and $lr\_w > 10^{-5}$}{
        Optimization $w$ with $\mathcal{L}$ in Eq.7 of $I$ and $G(W;\theta)$\;
        \If{the $\mathcal{L}$ ceases to decrease for five consecutive iterations}{
            $lr\_w = lr\_w / 2$;}
        }
}
\end{algorithm}
\end{comment}
\begin{algorithm}[t]
%\SetAlgoNoLine
\caption{Round-robin Optimization}
\label{alg:one}
\KwData{all codes $w \in W$ predicted by encoders, fixed GIRAFFE generator $G$, input image $I$;}
Initialize $lr\_w = 10^{-3} ,w\in W$ \;
\While{any $lr\_w > 10^{-5}$}{
     \ForEach{ $w \in W$}{
            Sample $\delta w$\;
            Compute $\delta \mathcal{L}(w)$ using Eq. \ref{Differential};
     }
     Compute $rank\_list$ using Eq. \ref{rank}\;
     \ForEach{ $w \in rank\_list$ and $lr\_w > 10^{-5}$}{
        Optimization $w$ with $\mathcal{L}_{opt}$ in Eq. \ref{loss_opt} of $I$ and $G(W;\theta)$\;
        \If{the $\mathcal{L}_{opt}$ ceases to decrease for five consecutive iterations}{
            $lr\_w = lr\_w / 2$;}
        }
}

\end{algorithm}


\begin{figure*}[!h]
%\setlength{\abovecaptionskip}{-0.1cm}
%\setlength{\belowcaptionskip}{-0.3cm}
\centering
\begin{subfigure}{0.23\linewidth}
\centering
\includegraphics[width=1\textwidth]{figures/single_car/recon.png}
    %\fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{\scriptsize Input,  Co-Recon,  Pre-Recon}
    % \label{fig:short-a}
\end{subfigure}
\hfill
\begin{subfigure}{0.23\linewidth}
\centering
\includegraphics[width=1\textwidth]{figures/single_car/shape.png}
    %\fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Edit Shape}
    % \label{fig:short-a}
\end{subfigure}
\hfill
\begin{subfigure}{0.23\linewidth}
\centering
\includegraphics[width=1\textwidth]{figures/single_car/app.png}
    %\fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Edit Appearance}
    % \label{fig:short-a}
\end{subfigure}
\hfill
\begin{subfigure}{0.23\linewidth}
\centering
\includegraphics[width=1\textwidth]{figures/single_car/bg_shape.png}
    %\fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Edit Bg Shape}
    % \label{fig:short-a}
\end{subfigure}
\hfill
\
        %这个回车键很重要 \quad也可以
\begin{subfigure}{0.23\linewidth}
\centering
\includegraphics[width=1\textwidth]{figures/single_car/bg_app.png}
    %\fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Edit Bg Appearance}
    % \label{fig:short-a}
\end{subfigure}
\hfill
\begin{subfigure}{0.23\linewidth}
\centering
\includegraphics[width=1\textwidth]{figures/single_car/scale.png}
    %\fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Edit Scale}
    % \label{fig:short-a}
\end{subfigure}
\hfill
\begin{subfigure}{0.23\linewidth}
\centering
\includegraphics[width=1\textwidth]{figures/single_car/trans.png}
    %\fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Edit Translation}
    % \label{fig:short-a}
\end{subfigure}
\hfill
\begin{subfigure}{0.23\linewidth}
\centering
\includegraphics[width=1\textwidth]{figures/single_car/rotation.png}
    %\fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Edit Rotation}
    % \label{fig:short-a}
\end{subfigure}
\hfill

\centering
\caption{ \scriptsize Single-object editing on \textit{G-CompCars} dataset. Co-Recon: coarse reconstruction. Pre-Recon: precise reconstruction.}
\vspace{-0.3cm}
\label{fig:single_car}
\end{figure*}

\begin{figure*}[!h]
%\setlength{\abovecaptionskip}{-0.1cm}
%\setlength{\belowcaptionskip}{-0.3cm}
\centering
\begin{subfigure}{0.23\linewidth}
\centering
\includegraphics[width=1\textwidth]{figures/single_clevr/reconstruction.jpg.png}
    %\fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{\scriptsize Input, Co-Recon, Pre-Recon}
    % \label{fig:short-a}
\end{subfigure}
\hfill
\begin{subfigure}{0.23\linewidth}
\centering
\includegraphics[width=1\textwidth]{figures/single_clevr/app.png}
    %\fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Edit Appearance}
    % \label{fig:short-a}
\end{subfigure}
\hfill
\begin{subfigure}{0.23\linewidth}
\centering
\includegraphics[width=1\textwidth]{figures/single_clevr/trans.png}
    %\fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Edit Translation}
    % \label{fig:short-a}
\end{subfigure}
\hfill
\begin{subfigure}{0.23\linewidth}
\centering
\includegraphics[width=1\textwidth]{figures/single_clevr/add.png}
    %\fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Add Object}
    % \label{fig:short-a}
\end{subfigure}
\hfill
\centering
\caption{\scriptsize Single-object editing on \textit{Clevr} dataset. }
\label{fig:single_clver}
\vspace{-0.3cm}
\end{figure*}

\begin{figure*}[!h]
\centering
\begin{subfigure}{0.23\linewidth}
\centering
\includegraphics[width=1\textwidth]{figures/multi_cars/recon.png}
    %\fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{\scriptsize Input,  Co-Recon,  Pre-Recon}
    % \label{fig:short-a}
\end{subfigure}
\hfill
\begin{subfigure}{0.23\linewidth}
\centering
\includegraphics[width=1\textwidth]{figures/multi_cars/shape.png}
    %\fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Edit Shape}
    % \label{fig:short-a}
\end{subfigure}
\hfill
\begin{subfigure}{0.23\linewidth}
\centering
\includegraphics[width=1\textwidth]{figures/multi_cars/app.png}
    %\fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Edit Appearance}
    % \label{fig:short-a}
\end{subfigure}
\hfill
\begin{subfigure}{0.23\linewidth}
\centering
\includegraphics[width=1\textwidth]{figures/multi_cars/bg_shape.png}
    %\fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Edit Bg Shape}
    % \label{fig:short-a}
\end{subfigure}
\hfill

\
        %这个回车键很重要 \quad也可以
\begin{subfigure}{0.23\linewidth}
\centering
\includegraphics[width=1\textwidth]{figures/multi_cars/bg_app.png}
    %\fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Edit Bg Appearance}
    % \label{fig:short-a}
\end{subfigure}
\hfill
\begin{subfigure}{0.23\linewidth}
\centering
\includegraphics[width=1\textwidth]{figures/multi_cars/scale.png}
    %\fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Edit Scale}
    % \label{fig:short-a}
\end{subfigure}
\hfill
\begin{subfigure}{0.23\linewidth}
\centering
\includegraphics[width=1\textwidth]{figures/multi_cars/trans.png}
    %\fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Edit Translation}
    % \label{fig:short-a}
\end{subfigure}
\hfill
\begin{subfigure}{0.23\linewidth}
\centering
\includegraphics[width=1\textwidth]{figures/multi_cars/rotation.png}
    %\fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Edit Rotation}
    % \label{fig:short-a}
\end{subfigure}
\hfill
\centering
\caption{\scriptsize Multi-object editing on \textit{G-CompCars} dataset.} 
\vspace{-0.3cm}
\label{fig:two_cars}
\end{figure*}

\begin{figure*}[!h]
%\setlength{\abovecaptionskip}{-0.1cm}
%\setlength{\belowcaptionskip}{-0.3cm}
\centering
\begin{subfigure}{0.23\linewidth}
\centering
\includegraphics[width=1\textwidth]{figures/multi_clevrs/recon.png}
    %\fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{\scriptsize Input, Co-Recon,  Pre-Recon}
    % \label{fig:short-a}
\end{subfigure}
\hfill
\begin{subfigure}{0.23\linewidth}
\centering
\includegraphics[width=1\textwidth]{figures/multi_clevrs/app.png}
    %\fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Edit Appearance}
    % \label{fig:short-a}
\end{subfigure}
\hfill
\begin{subfigure}{0.23\linewidth}
\centering
\includegraphics[width=1\textwidth]{figures/multi_clevrs/trans.png}
    %\fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Edit Translation}
    % \label{fig:short-a}
\end{subfigure}
\hfill
\begin{subfigure}{0.23\linewidth}
\centering
\includegraphics[width=1\textwidth]{figures/multi_clevrs/add.png}
    %\fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{\scriptsize Add or Remove Objects}
    % \label{fig:short-a}
\end{subfigure}
\hfill
\centering
\caption{\scriptsize Multi-object editing on \textit{Clevr} dataset. }
\label{fig:multi_clver}
\vspace{-0.3cm}
\end{figure*}



\subsection{Precise Optimization}

\label{sec:4.4}
Next, we optimize the coarse codes predicted by the encoder. Through experiments, we have found that using a single optimizer to simultaneously optimize all latent codes tends to converge to local minima. To circumvent this, we employ multiple optimizers, each handling a single code as in the coarse estimation. The optimization order plays a crucial role in the overall outcome due to the variance of the disparity between the predicted and actual values across different encoders, and the different impact of code changes on the image, e.g., changes to  $bg\_shape$ and $bg\_app$ codes controlling background generation mostly would have a larger impact on overall pixel values. Prioritizing the optimization of codes with significant disparity and a high potential for changing pixel values tends to yield superior results in our empirical experiments. Hence, we propose an automated round-robin optimization algorithm (Algorithm~\ref{alg:one}) to sequentially optimize each code based on the image reconstructed in each round.

\par Algorithm~\ref{alg:one} aims to add multiple minor disturbances to each code, and calculate the loss between the images reconstructed before and after the disturbance and the original image. A loss increase indicates that the current code value is relatively accurate, hence its optimization order can be put later. A loss decrease indicates that the current code value is inaccurate and thus should be prioritized. For multiple codes that demand prioritized optimization, we compute their priorities using the partial derivatives of the loss variation and perturbation. We do not use backpropagation automatic differentiation here to ensure the current code value remains unchanged. %Using automatic differentiation would change the code value.).%这里不使用反向传播自动微分是因为，在评估优化顺序的时候我们要保证当前的code值不变，使用自动微分后就会改变code的值
\begin{equation}
    \delta \mathcal{L}(w) = \mathcal{L}(G(W-\{w\},w+\delta w,\theta),I)-\mathcal{L}
   (G(W,\theta),I) \label{Differential} ,
\end{equation}
\begin{equation}
    rank\_list = F_{rank}( \delta \mathcal{L}(w),\frac{ \delta \mathcal{L}(w)}{\delta w}) ,  \label{rank}
\end{equation}
where $w \in W$ is one of the codes and $\delta w$ represents the minor disturbance of $w$. For the rotation angle $r$, we have found that adding a depth loss can accelerate its optimization. 
%We chose not to include it in the encoder because its inclusion tends to slow down the training speed and doesn't significantly impact the results. 
Therefore, the loss $\mathcal{L}$ during the optimization stage can be expressed as:
\begin{equation}
    \mathcal{L}_{opt} = \lambda_1 L_2 + \lambda_2 L_{lpips} + \lambda_3 L_{id} + \lambda_4 L_{deep}. \label{loss_opt}
\end{equation}
\par This optimization method allows for more precise tuning of the codes for more accurate reconstruction and editing of the images.
%By optimizing the codes separately, we can better manage the complexity and dependencies of the latent space, allowing for more effective and flexible image editing.














==> supp_bbl.tex <==
\begin{thebibliography}{10}
\providecommand{\url}[1]{\texttt{#1}}
\providecommand{\urlprefix}{URL }
\providecommand{\doi}[1]{https://doi.org/#1}

\bibitem{alaluf2022hyperstyle}
Alaluf, Y., Tov, O., Mokady, R., Gal, R., Bermano, A.: Hyperstyle: Stylegan inversion with hypernetworks for real image editing. In: Proceedings of the IEEE/CVF conference on computer Vision and pattern recognition. pp. 18511--18521 (2022)

\bibitem{bhattarai2023triplanenet}
Bhattarai, A.R., Nie{\ss}ner, M., Sevastopolsky, A.: Triplanenet: An encoder for eg3d inversion. arXiv preprint arXiv:2303.13497  (2023)

\bibitem{chan2022efficient}
Chan, E.R., Lin, C.Z., Chan, M.A., Nagano, K., Pan, B., De~Mello, S., Gallo, O., Guibas, L.J., Tremblay, J., Khamis, S., et~al.: Efficient geometry-aware 3d generative adversarial networks. In: Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition. pp. 16123--16133 (2022)

\bibitem{karras2020analyzing}
Karras, T., Laine, S., Aittala, M., Hellsten, J., Lehtinen, J., Aila, T.: Analyzing and improving the image quality of stylegan. In: Proceedings of the IEEE/CVF conference on computer vision and pattern recognition. pp. 8110--8119 (2020)

\bibitem{lan2023self}
Lan, Y., Meng, X., Yang, S., Loy, C.C., Dai, B.: Self-supervised geometry-aware encoder for style-based 3d gan inversion. In: Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition. pp. 20940--20949 (2023)

\bibitem{mildenhall2021nerf}
Mildenhall, B., Srinivasan, P.P., Tancik, M., Barron, J.T., Ramamoorthi, R., Ng, R.: Nerf: Representing scenes as neural radiance fields for view synthesis. Communications of the ACM  \textbf{65}(1),  99--106 (2021)

\bibitem{niemeyer2021giraffe}
Niemeyer, M., Geiger, A.: Giraffe: Representing scenes as compositional generative neural feature fields. In: Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition. pp. 11453--11464 (2021)

\bibitem{richardson2021encoding}
Richardson, E., Alaluf, Y., Patashnik, O., Nitzan, Y., Azar, Y., Shapiro, S., Cohen-Or, D.: Encoding in style: a stylegan encoder for image-to-image translation. In: Proceedings of the IEEE/CVF conference on computer vision and pattern recognition. pp. 2287--2296 (2021)

\bibitem{roich2022pivotal}
Roich, D., Mokady, R., Bermano, A.H., Cohen-Or, D.: Pivotal tuning for latent-based editing of real images. ACM Transactions on Graphics (TOG)  \textbf{42}(1),  1--13 (2022)

\bibitem{schwarz2020graf}
Schwarz, K., Liao, Y., Niemeyer, M., Geiger, A.: Graf: Generative radiance fields for 3d-aware image synthesis. Advances in Neural Information Processing Systems  \textbf{33},  20154--20166 (2020)

\bibitem{tov2021designing}
Tov, O., Alaluf, Y., Nitzan, Y., Patashnik, O., Cohen-Or, D.: Designing an encoder for stylegan image manipulation. ACM Transactions on Graphics (TOG)  \textbf{40}(4),  1--14 (2021)

\bibitem{wang2022high}
Wang, T., Zhang, Y., Fan, Y., Wang, J., Chen, Q.: High-fidelity gan inversion for image attribute editing. In: Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition. pp. 11379--11388 (2022)

\bibitem{yin20223d}
Yin, F., Zhang, Y., Wang, X., Wang, T., Li, X., Gong, Y., Fan, Y., Cun, X., Shan, Y., Oztireli, C., et~al.: 3d gan inversion with facial symmetry prior. arXiv preprint arXiv:2211.16927  (2022)

\end{thebibliography}

